Tactile Object Pose Estimation from the First Touch with Geometric Contact Rendering

In this paper, we present an approach to tactile pose estimation from the first touch for known objects. First, we create an object-agnostic map from real tactile observations to contact shapes. Next, for a new object with known geometry, we learn a tailored perception model completely in simulation. To do so, we simulate the contact shapes that a dense set of object poses would produce on the sensor. Then, given a new contact shape obtained from the sensor output, we match it against the pre-computed set using the object-specific embedding learned purely in simulation using contrastive learning. This results in a perception model that can localize objects from a single tactile observation. It also allows reasoning over pose distributions and including additional pose constraints coming from other perception systems or multiple contacts. We provide quantitative results for four objects. Our approach provides high accuracy pose estimations from distinctive tactile observations while regressing pose distributions to account for those contact shapes that could result from different object poses. We further extend and test our approach in multi-contact scenarios where several tactile sensors are simultaneously in contact with the object. Website: http://mcube.mit.edu/research/tactile_loc_first_touch.html

==> preliminaries.tex <==
\vspace{-2mm}
\section{Preliminaries}
\vspace{-3mm}
In visual MPC (or visual foresight), the robot first collects a dataset $D = \{\tau^{(1)}, \tau^{(2)}, ..., \tau^{(N)}\}$ which contains $N$ trajectories.
%
Each trajectory $\tau$ can further be represented as a sequence of images and actions $\tau = \{I_1, a_1, I_2, a_2, ..., I_T\}$.
%
%
Then, the dataset is used to learn an action-conditioned video prediction model $g_{\theta}$ that approximates the stochastic visual dynamics $p(I_{t}|I_{1:t-1}, a_{t-1})$.
%
Once the model is learned, it can be coupled with a planner to find actions that minimize an objective specified by user.
%
In this work, we adopt the cross entropy method (CEM) as our planner and assume the objective is specified as a goal image. 
%
At the planning stage, CEM aims to find a sequence of actions that minimizes the difference between the predicted future frames and the goal image.
%
Then, the robot executes the first action in the planned action sequence and performs replanning.
%
